The Contact and Mobility Networks of Mexico City

Mexico City, the largest city in Mexico, is also one of the largest cities in the world. It has over 9 million inhabitants and concentrates the vast majority of government and business centers. In this work we describe algorithms that use anonymized location data from mobile devices to construct Mexico City's contact and mobility networks aiming to help the analysis of the city's complexity by understanding movement and physical interaction patterns between its inhabitants. We show the effectiveness and usefulness of our approach by building networks with data collected in February 2020 and performing a general descriptive analysis on them. We found that contact networks in Mexico City are very sparse, characterized by a largest connected component, and with a heavy-tailed degree distribution. On the other hand, we observed that paths conformed by the highest-degrree nodes of mobility networks resemble Mexico City's street network; moreover, we found interesting qualitative differences in the degree distribution of these networks between weekends and weekdays. We present these results along with the release of contact and mobility networks.

==> backup_Bibitems.tex <==
\begin{thebibliography}
\bibitem{Farmer1990}
J~Doyne Farmer.
\newblock A rosetta stone for connectionism.
\newblock {\em Physica D: Nonlinear Phenomena}, 42(1-3):153--187, 1990.

\bibitem{Pflieger2010}
Géraldine Pflieger and Céline Rozenblat.
\newblock Introduction. urban networks and network theory: The city as the
  connector of multiple networks.
\newblock {\em Urban Studies}, 47(13):2723--2735, 2010.

\bibitem{Barthelemy2019}
Marc Barthelemy.
\newblock The statistical physics of cities.
\newblock {\em Nature Reviews Physics}, 1(6):406–415, May 2019.

\bibitem{Gallotti2019}
Riccardo Gallotti, Giulia Bertagnolli, and Manlio~De Domenico.
\newblock Disentangling activity-aware human flows reveals the hidden
  functional organization of urban systems.
\newblock {\em arXiv}, 2019.
\newblock https://arxiv.org/abs/1908.02538.

\bibitem{Barrat2008}
Alain Barrat, Ciro Cattuto, Vittoria Colizza, {Jean-François} Pinton, Wouter
  {Van den Broeck}, and Alessandro Vespignani.
\newblock High resolution dynamical mapping of social interactions with active
  rfid.
\newblock {\em ArXiv e-prints}, November 2008.

\bibitem{Huang2015}
Xiaoke Huang, Ye~Zhao, Chao Ma, Jing Yang, Xinyue Ye, and Chong Zhang.
\newblock Trajgraph: A graph-based visual analytics approach to studying urban
  network centralities using taxi trajectory data.
\newblock {\em IEEE transactions on visualization and computer graphics},
  22(1):160--169, 2015.

\bibitem{Yildirimoglu2018}
Mehmet Yildirimoglu and Jiwon Kim.
\newblock Identification of communities in urban mobility networks using
  multi-layer graphs of network traffic.
\newblock {\em Transportation Research Part C: Emerging Technologies},
  89:254--267, 2018.

\bibitem{Liu2015}
Xi~Liu, Li~Gong, Yongxi Gong, and Yu~Liu.
\newblock Revealing travel patterns and city structure with taxi trip data.
\newblock {\em Journal of Transport Geography}, 43:78--90, 2015.

\bibitem{Du2017}
Zhanwei Du, Bo~Yang, and Jiming Liu.
\newblock Understanding the spatial and temporal activity patterns of subway
  mobility flows.
\newblock {\em arXiv preprint arXiv:1702.02456}, 2017.

\bibitem{Zhong2015}
Chen Zhong, Ed~Manley, Stefan~Mueller Arisona, Michael Batty, and Gerhard
  Schmitt.
\newblock Measuring variability of mobility patterns from multiday smart-card
  data.
\newblock {\em Journal of Computational Science}, 9:125--130, 2015.

%doi:10.1559/152304003100011090
\bibitem{Sahr2003}
Kevin Sahr, Denis White, and A.~Jon Kimerling.
\newblock Geodesic discrete global grid systems.
\newblock {\em Cartography and Geographic Information Science}, 30(2):121--134,
  2003.

\bibitem{Clauset2009}
Aaron Clauset, Cosma~Rohilla Shalizi, and M.~E.~J. Newman.
\newblock Power-law distributions in empirical data.
\newblock {\em SIAM Review}, 51(4):661–703, November 2009.

\bibitem{Sapiezynski2019}
Piotr Sapiezynski, Arkadiusz Stopczynski, David~Dreyer Lassen, and Sune
  Lehmann.
\newblock Interaction data from the copenhagen networks study.
\newblock {\em Scientific Data}, 6(1), December 2019.
\end{thebibliography}

